GoalNet: Inferring Conjunctive Goal Predicates from Human Plan Demonstrations for Robot Instruction Following

Our goal is to enable a robot to learn how to sequence its actions to perform tasks specified as natural language instructions, given successful demonstrations from a human partner. The ability to plan high-level tasks can be factored as (i) inferring specific goal predicates that characterize the task implied by a language instruction for a given world state and (ii) synthesizing a feasible goal-reaching action-sequence with such predicates. For the former, we leverage a neural network prediction model, while utilizing a symbolic planner for the latter. We introduce a novel neuro-symbolic model, GoalNet, for contextual and task dependent inference of goal predicates from human demonstrations and linguistic task descriptions. GoalNet combines (i) learning, where dense representations are acquired for language instruction and the world state that enables generalization to novel settings and (ii) planning, where the cause-effect modeling by the symbolic planner eschews irrelevant predicates facilitating multi-stage decision making in large domains. GoalNet demonstrates a significant improvement (51%) in the task completion rate in comparison to a state-of-the-art rule-based approach on a benchmark data set displaying linguistic variations, particularly for multi-stage instructions.

==> results.tex <==
\section{Evaluation and Results}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/frequency.pdf}
    \caption{Dataset characteristics. Frequency of plans with plan length.}
    \label{fig:freq}
\end{figure}

% Experimentation setup and model training details
\noindent \textbf{Data set and Training.}
\\
We have used the same train, validation and test split from \citep{She2016IncrementalAO}(779 train, 157 validation and 181 test instances). Data augmentation on train set using object replacements increased our total train set size to 960 instances.
\\
Each instruction with a single verb can be completed by one or multiple actions. Average action length is 4.9 for both train and test set. 
\\
There are 2 domains in the dataset, kitchen and living room, each containing 40 objects. Using different configurations of the objects,there are 453 unique initial states in train set, 106 in val set and 109 in test set. Total of test and train set has 562 unique initial states, showing no overlap in train and test initial states. The instructions varies from low level task like, \emph{``go to the sink"} to high level tasks like \emph{``cook the ramen in the pot with water"}. See Table \ref{tab:Objects} for a list of domain objects, their states and  properties and robot symbolic actions.

The model is trained for 100 epochs. Best model is choosen based on validation set accuracy.
%
Learning rate of 0.0005 is used with a stepwise LR decay scheduler and Adam optimizer. We use teacher forcing during training to improve model skill and stability when training. Teacher forcing is gradually removed with increase in epochs. 
%

During training we use a lexical planner to optimize training time. This lexical planner updates the current state by adding predicted  positive constraint and removing predicted negative constraint. However to get best results, we use \textsc{Rintanen} \citep{RINTANEN201245} during inference. This symbolic planner is able to predict actions and update environment state with action effects and side effects, providing complete update of env state.
%

\modelname predicts actions and predicated in a recurrent manner,stopping when the predicted predicate pos. and neg. are both zero or till a maximum of 30 predictions. This number is chosen empirically from the maximum plan lengths in test and train set.

\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}p{1.4\linewidth}@{}}
    \toprule
    \textbf{Objects in kitchen}\tabularnewline
    \midrule
    Sink, Stove, Mug, , Microwave, Fridge, IceCream, Kettle, Coke,  Plate, BoiledEgg, Salt,  StoveFire,  SinkKnob,  \tabularnewline
    \midrule
    \textbf{Objects in living room}\tabularnewline
    \midrule
   Loveseat, Armchair,  CoffeeTable, Tv,  Pillow,  BagOfChips, Bowl, GarbageBag, Shelf, Book, Coke, Beer,  Xbox, Cd 
    \tabularnewline
    \midrule
    \textbf{Objects states}\tabularnewline
    \midrule
  IsOpen, MicrowaveIsOn,  LeftDoorIsOpen, IsOn, Water,  TapIsOn, HasChips, RightDoorIsOpen, DoorIsOpen \tabularnewline
  \midrule
    \textbf{Objects properties}\tabularnewline
    \midrule
 IsPlaceableOn, Turnable, IsGraspable, Pressable, IsTurnable, IsAddable, IsSqueezeable, IsPlaceableIn, Openable \tabularnewline
 \midrule
    \textbf{Robot symbolic actions }\tabularnewline
    \midrule
 grasp, release, moveto, press, turn, open, close , keep, pour, add, squeeze, scoop, place, insert\tabularnewline
 \midrule
    \textbf{All predicates}\tabularnewline
    \midrule
    (state $o_1$ ??),(Grasping Robot $o_1$),(Near Robot $o_1$),(In $o_1$ $o_2$),(On $o_1$ $o_2$)
  \tabularnewline
 \midrule
    \textbf{Robot symbolic actions }\tabularnewline
    \midrule
 grasp, release, moveto, press, turn, open, close , keep, pour, add, squeeze, scoop, place, insert\tabularnewline
   \bottomrule
    \end{tabular}
    }
    \caption{Domain objects, states and properties,robot symbolic actions(complete list in appendix)}
    \label{tab:Objects}
\end{table}


% Describe baseline model and metrics.
\subsection{Baselines and Metrics}
We adopt the approach by Chai et al. as the baseline. 
The approach addresses the problem of inferring a hypothesis space 
for verb frames extracted from language instructions. 
%
The determination of hypothesis space uses heuristics to focus the learner 
only on a focused set of predicates. 
%
Further, hand-crafted features extracted from
language instruction, world state and the candidate goal states is used during 
learning. 
%
A log-linear model is then trained incrementally with successful demonstration of a plan.
%
We adopt this model as a baseline and compare the approach in a batch (instead of and incremental) setting. {\color{red}Need to add why we choose 2016 model as baseline and what about latest works}
%

The following metrics are used to evaluate the approach. The metrics evaluate 
aspects such as the ability to reconstruct the set of goal constraints 
(at the end of the instruction) and nearness of the estimated plan in relation to the human demonstration. 
%
We adopt the state jaccard index and instruction edit distance measures from the baseline \cite{}. In addition, we also report the F-measures and Goal Reaching Rate (GRR) score computed from the predicted constraint sets.  
%
Formally, the metrics are computed as: 
\begin{itemize}
    \item SJI
    \item IED
    \item GRR
    \item F-measure
\end{itemize}

% Comparison with baselines
\subsection{Baseline Comparison}
Table \ref{tab:Comparison with baselines and ablation} presents the results of our model \modelname and compares it with \citep{She2016IncrementalAO}. For a fair comparison, we
consider the grounding-aware version of the model where
the instance grounding for a noun is assumed known from the dataset. For instance,objects like counter and pot are grounded to \emph{"counter\_1"} and \emph{"Kettle"} respectively in the instruction \emph{"take pot on counter"}. We are able to achieve 25\% improvement in SJI and 33\% improvement in IED. Robot is able to reach to final goal state in 84 cases in \modelname vs 66 vases in \citep{She2016IncrementalAO} out of 181 test data points. Learning dense representation of world state, state history and language instruction enables \modelname to generalize to settings not encountered during training and perform better than hand crafted feature approach of \citep{She2016IncrementalAO}.
%

%
\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lcccccc@{}}
    \toprule
    \textbf{Model} & \textbf{SJI} & \textbf{IED} & \textbf{F1} & \textbf{GRR}\tabularnewline
    \midrule
    Baseline \citep{She2016IncrementalAO} & 0.448  &  0.450 & 0.512 & 0.370 
 \tabularnewline
    \midrule
    \modelname &0.562  &0.601  &0.651  &0.468 \tabularnewline
    \midrule
    \textbf{Model Ablations} \tabularnewline
    \midrule
   - Relational information encoding&0.533 &0.575 &0.621 &0.449\tabularnewline
   - Instance Grounding &0.528 &0.567 &0.617 &0.439\tabularnewline
    - Negative Constraint prediction &0.424  &0.447 &0.533 &0.416\tabularnewline
    - Positive constraint prediction &0.156 &0.167 &0.195 &0.098\tabularnewline
    - Constraint History encoding &0.221  &0.323  &0.263   &0.159 \tabularnewline
    - State conditioned Self-Attn &0.547  &0.595   &0.634  &0.430 \tabularnewline
    - Instruction conditioned Attn &0.565  &0.604  &0.650  &0.456 \tabularnewline
    - Instruction objects encoding &0.532  &0.568  &0.616  &0.435 \tabularnewline
    - Grammar mask &0.567  &0.602  &0.651  &0.459 \tabularnewline
    \midrule
    \textbf{Model Explorations} \tabularnewline
    \midrule
    Instruction encoding : Conceptnet &0.389  &0.451  &0.477  &0.297 \tabularnewline
    \midrule
     Constraint History($\delta^+_{t-1} \cup \delta^-_{t-1}$) &0.552 &0.580 &0.637 &0.430 \tabularnewline
    Constraint History($s_{t+1}$) &0.503 &0.553 &0.593 &0.380 \tabularnewline
    \midrule
    Symbolic planner : 
    \textsc{Rintanen} &\textbf{0.645}  &\textbf{0.661}  &\textbf{0.717}  &\textbf{0.558} \tabularnewline
    \bottomrule
    \end{tabular}
    }
    \caption{A comparison of goal-prediction and goal reaching performance for the baseline, the proposed \modelname model, ablations and explorations. Results are presented for test set derived from living room and kitchen domains.}
    \label{tab:Comparison with baselines and ablation}
\end{table}
%


%% Model Components
\subsection{Analysis of Model Components}
In this section, we analyse the importance of model components by performing an ablation study. Table \ref{tab:Comparison with baselines and ablation} (lower
half) presents the results. For a fair comparison, the model
capacities remain the same during the ablation experiments.

%
%Relational information
\modelname represents relations of each object with as a adjacency vector, which is then encoded using a FCN. Late fusion of this relational information with semantic information provides a better performance as the model is now aware of objects relations also along with objects states and properties. For instruction like \emph{"arrange all pillows on shelf"}, \modelname will already be aware which pillows are already present on shelf and will not predict those actions, resulting in a better IED. We will further explore use of relational information using a Graph Neural Network \citep{DBLP:journals/corr/abs-1812-08434} as a future direction to this work.

% Use of instance grounding
\citep{She2016IncrementalAO} dataset provides instance grounding of objects in the instruction. The instance mappings are densely encoded using $\mathrm{ConceptNet}$ \citep{conceptnet-github}. These embeddings are then appended to the set of objects in the instruction $O_l$. This combined embedding is then used to generate the encoding of the objects in the instruction using Bahdanau style state-conditioned self-attention \citep{bahdanau2014neural}. Removing information of instance grounding from the dataset reduces the SJI and IED score by ~6\%. This reduction is expected as use of instance grounding provides a more informed signal for predicting correct objects in goal constraints.
However, it should be noted that without this instance grounding also, \modelname still performs better than \citep{She2016IncrementalAO}, as \modelname performs automatic extraction of object nouns from the instruction using NLTK tokeniser. For instance, in the instruction \emph{”take pot on counter”}, NLTK tokeniser \citep{bird2009natural} automatically extracts \emph{“pot"} and \emph{“counter”} and uses $\mathrm{ConceptNet}$ \citep{conceptnet-github} to encode these objects.

% Use of State conditioned self-attention
In a single instruction, robot can manipulate multiple objects. Since our model recurrently predicts the constraints, it is important to know the state of the environment and attend on goal objects based on current environment state. As an ablation experiment, we removed the attention on goal objects and replaced it with an equal weighted average of all objects tokens and instance groundings. This led to slight decrease in SJI and IED with ~8\% drop in task completion rate.

%Use of Goal Objects
If we remove the overall embedding ($\tilde{l}_{obj}$) of goal objects from $f_\theta^{goal}$, it further reduces the final SJI and IED values, putting  more emphasis on the importance of goal objects embeddings in predicting the correct objects. For instruction, \emph{"take pillows from shelf"}, \modelname correctly identifies all 3 pillow instances and predicts following goal constraint - \emph{'(near robot armchair\_1)', '(grasping robot pillow\_1)', '(near robot armchair\_2)', '(grasping robot pillow\_3)', '(grasping robot pillow\_2)'}. However the model without ($\tilde{l}_{obj}$) is sometimes unable to ground to all instances. For same instruction as above, this model is unable to ground $pillow\_2$ and predicts the following goal constraint \emph{'(on garbagebag\_1 loveseat\_1)', '(grasping robot pillow\_1)', '(grasping robot pillow\_3)'}

%Use of instruction conditioned attention
We use language instruction encoding $\tilde{l}$ to attend over the world objects. The attention operation aligns the information of the input language sentence with the scene to learn task-relevant context by allocating appropriate weights to objects. However, for this data set, it is observed that this attention does not provide any significant improvement in performance. This may be due to the fact that we are already encoding goal objects information separately as ($\tilde{l}_{obj}$), which is sending relevant information to downstream predictors about required goal objects. This attention might be particularly helpful in the absence of instance groundings for instructions like, \emph{“Bring all utensils to sink”}. In such cases, tokeniser will only extract \emph{“utensils”}, which will not be mapped directly to any object in the environment and ($\tilde{l}_{obj}$) might not provide relevant information. In such cases, if instruction is used to attend over environment, due to word embeddings closeness, objects like \emph{“Plate”}, \emph{“Spoon”} can get high attention weights.
 
%Use of delta positive and negative constraints
When we remove the negative constraint predictor, SJI and IED drops by ~24\% . This reduction is expected as the model is not predicting complete output now. However the performance is still close enough to \cite{She2016IncrementalAO} , with SJI and IED being marginally worse and F1 and GRR being better.
However removing the positive constraint predictor completely drops the performance, as negative constraints only does not contain enough information for the robot to perform actions. 

%Grammar mask
A mask $\Lambda$ is applied at inference time to impose grammar constraints. In the absence of this graph, the performance of final model remains similar. This highlights that the model is able to learn the grammar constraints on its own. During initial epochs, the model predicts few inconsistent states of objects, which gets corrected later as the training progresses. During inference, such inconsistent states are not observed at all, resulting in similar performance to \modelname.

\begin{figure*}
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/fill_kettle/1.png} \vspace{-16pt}
        \caption{Initial State} \vspace{-6pt}
        \label{fig:fill_kettle_1}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/fill_kettle/2.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{ConnectedTo(mug_0, robot)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, mug_0)}$, $\mathrm{Grasp(robot, mug_0)}$\}} \vspace{-6pt}
        \label{fig:fill_kettle_2}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/fill_kettle/4.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{Near(robot, sink_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, sink_0)}$\}} \vspace{-6pt}
        \label{fig:fill_kettle_4}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/fill_kettle/3.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{OnTop(mug_0, sink_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{PlaceOn(mug_0, sink_0)}$\}} \vspace{-6pt}
        \label{fig:fill_kettle_3}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/fill_kettle/5.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{stateIsOn(tap_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{stateOn(tap_0)}$\}} \vspace{-6pt}
        \label{fig:fill_kettle_5}
    \end{subfigure}
    \caption{Execution of \textit{``fill water in mug''} by \modelname.  }
    \label{fig:fill_kettle}
\end{figure*}

\begin{figure*}
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/heat_milk/1.png} \vspace{-16pt}
        \caption{Initial State} \vspace{-6pt}
        \label{fig:heat_milk_1}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/heat_milk/2.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{stateIsOpen(microwave_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, microwave_0)}$, $\mathrm{stateOpen(microwave_0)}$\}} \vspace{-6pt}
        \label{fig:heat_milk_2}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/heat_milk/3.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{ConnectedTo(milk_0, robot)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, milk_0)}$, $\mathrm{Grasp(robot, microwave_0)}$\}} \vspace{-6pt}
        \label{fig:heat_milk_3}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/heat_milk/4.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{Inside(milk_0, microwave_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, microwave_0)}$, $\mathrm{PlaceIn(milk_0, microwave_0)}$\}} \vspace{-6pt}
        \label{fig:heat_milk_4}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/heat_milk/5.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{stateIsOn(microwave_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{stateOn(microwave_0)}$\}} \vspace{-6pt}
        \label{fig:heat_milk_5}
    \end{subfigure}
    \caption{Execution of \textit{``heat milk''} by \modelname.}
    \label{fig:heat_milk}
\end{figure*}


\begin{figure*}
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_milk/1.png} \vspace{-16pt}
        \caption{Initial State} \vspace{-6pt}
        \label{fig:get_milk_1}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_milk/2.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{stateIsOpen(fridge_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, fridge_0)}$, $\mathrm{stateOpen(fridge_0)}$\}} \vspace{-6pt}
        \label{fig:get_milk_2}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_milk/3.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{ConnectedTo(milk_0, robot)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, milk_0)}$, $\mathrm{Grasp(robot, milk_0)}$\}} \vspace{-6pt}
        \label{fig:get_milk_3}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_milk/4.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{OnTop(milk_0, counter_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, counter_0)}$, $\mathrm{PlaceOn(milk_0, counter_0)}$\}} \vspace{-6pt}
        \label{fig:get_milk_4}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_milk/5.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{stateIsClose(fridge_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, fridge_0)}$, $\mathrm{stateClose(fridge_0)}$\}} \vspace{-6pt}
        \label{fig:get_milk_5}
    \end{subfigure}
    \caption{Execution of \textit{``get milk from fridge''} by \modelname.}
    \label{fig:get_milk}
\end{figure*}

\begin{figure*}
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_pillows/1.png} \vspace{-16pt}
        \caption{Initial State} \vspace{-6pt}
        \label{fig:get_pillows_1}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_pillows/2.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{ConnectedTo(pillow_0, robot)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, pillow_0)}$, $\mathrm{Grasp(robot, pillow_0)}$\}} \vspace{-6pt}
        \label{fig:get_pillows_2}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_pillows/3.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{OnTop(pillow_0, table_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, table_0)}$, $\mathrm{PlaceOn(pillow_0, table_0)}$\}} \vspace{-6pt}
        \label{fig:get_pillows_3}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_pillows/4.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{ConnectedTo(pillow_1, robot)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, pillow_1)}$, $\mathrm{Grasp(robot, pillow_1)}$\}} \vspace{-6pt}
        \label{fig:get_pillows_4}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_pillows/5.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{OnTop(pillow_1, table_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, table_0)}$, $\mathrm{PlaceOn(pillow_1, table_0)}$\}} \vspace{-6pt}
        \label{fig:get_pillows_5}
    \end{subfigure}
    \caption{Execution of \textit{``fetch pillows''} by \modelname.}
    \label{fig:get_pillows}
\end{figure*}

\begin{figure*}
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_beer_and_wine/1.png} \vspace{-16pt}
        \caption{Initial State} \vspace{-6pt}
        \label{fig:get_beer_and_wine_1}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_beer_and_wine/2.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{ConnectedTo(beer_0, robot)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, beer_0)}$, $\mathrm{Grasp(robot, beer_0)}$\}} \vspace{-6pt}
        \label{fig:get_beer_and_wine_2}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_beer_and_wine/3.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{OnTop(beer_0, table_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, table_0)}$, $\mathrm{PlaceOn(beer_0, table_0)}$\}} \vspace{-6pt}
        \label{fig:get_beer_and_wine_3}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_beer_and_wine/4.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{ConnectedTo(wine_0, robot)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, wine_0)}$, $\mathrm{Grasp(robot, wine_0)}$\}} \vspace{-6pt}
        \label{fig:get_beer_and_wine_4}
    \end{subfigure}
    \begin{subfigure}[t]{0.196\linewidth}
        \centering
        \includegraphics[width=\linewidth, height=0.7\linewidth]{figures/get_beer_and_wine/5.png} \vspace{-16pt}
        \caption{
        \scriptsize \red{$\mathrm{OnTop(wine_0, table_0)}$}}\\
        \scriptsize \blue{\{$\mathrm{MoveTo(robot, table_0)}$, $\mathrm{PlaceOn(wine_0, table_0)}$\}} \vspace{-6pt}
        \label{fig:get_beer_and_wine_5}
    \end{subfigure}
    \caption{Execution of \textit{``place beer and wine on top of the coffee-table''} by \modelname.}
    \label{fig:get_beer_and_wine}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.22\linewidth]{figures/sensitivity/legend.pdf}\\
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/sensitivity/SJI.pdf}
        \caption{SJI Score} \vspace{-6pt}
        \label{fig:sens_sji}
    \end{subfigure}\ \ 
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/sensitivity/IED.pdf}
        \caption{IED Score} \vspace{-6pt}
        \label{fig:sens_ied}
    \end{subfigure}\ \ 
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/sensitivity/F1.pdf}
        \caption{F1 Score} \vspace{-6pt}
        \label{fig:sens_f1}
    \end{subfigure}\ \ 
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/sensitivity/GRR.pdf}
        \caption{GRR Score} \vspace{-6pt}
        \label{fig:sens_grr}
    \end{subfigure}
    \caption{{\color{red}Sensitivity Analysis} of the performance of baseline and \modelname model with the size of overall goal-constraint set.}
    \label{fig:sensitivity}
\end{figure*}

\subsubsection{Effect of state history encoding}
This is one of the most important component of our model. In the absence of  constraint history encoding, model has no information of previously predicted constraints and is unable to predict multiple constraints needed to reach the final goal state.

The proposed model uses a temporal contextual history of only the positive constraints; however, when we also encode the history of predicted negative constraints (using another LSTM model) the task completion rate drops by 8\% as shown in Table \ref{tab:Comparison with baselines and ablation}
Using the complete update environment state further dropped the task completion rate by 19\%. This is due to the fact that when using complete environment state, the information of the last predicted constraint is lost complete as compared to sending just the last predicted constraint where it is a more focused information.

\subsubsection{Symbolic planner variation}
For the proposed model, we use a simple lexical planner in training, where the predicted constraints are just added and subtracted to create a new state. We also performed one experiment using Madagascar planner,  where predicted constraint are sent to Madagascar planner which in turns returns actions and final states. Due to limited time available, we have used a hybrid approach, where for first 50 epochs, we have used lexical planner and for next 15 epochs using \textsc{Rintanen} planner. This approach took 39 hours to train on vs 3 hours of using lexical planner for 100 epoch on same hardware. Hence for all ablations and explorations, we have used the model with lexical planner. The best performance is however achieved by using \textsc{Rintanen} \citep{RINTANEN201245} planner as it correctly gives the final state vs approximate state of lexical planner.
%
In all our model inference, we have used \textsc{Rintanen}. To show the importance of symbolic planner we also did inference without it using lexical planner only. This resulted in IED score of '0' as no planner to predict actions. SJI- 0.264, GRR - 0.16, F1- 0.379.

Lastly, we replaced Sbert with BoW of Conceptnet embeddings. The performance drops from SJI 0.562 to 0.389. This highlights the power of pre-trained language models like BERT and their ability to encode sequences.

{\color{red}
\subsubsection{Use of GNN for world encoding}
...
}

\subsubsection{Qualitative Analysis}
\begin{itemize}
\item Figure \ref{fig:sensitivity} shows the variation of SJI, IED, F1 and GRR with size of total ground truth constraint set (($len(\delta^+) + len(\delta^-)$).  We observed graceful degradation in performance as constraint length increases showing that the model still needs improvement on the large constraint length predictions. However, it should be observed that performance of \modelname is better than \cite{She2016IncrementalAO} for all size of goal constraint set. The performance gap is more significant for the larger constraint sets, showing that the neural approach in \modelname is able to generalize better for longer instructions also.
{\color{red}check discrepancy for constraint len = 5}
\item Figure \ref{fig:Results}, shows goal constraints inferred for instructions in the test set and compares those with \citep{She2016IncrementalAO}
\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/QualitativeAnalysis.pdf}
    \caption{Comparison of \modelname output with ACL}
    \label{fig:Results}
\end{figure*}

\subsection{Generalization}
We developed two generalization datasets for objects and verbs separately to show how well our neuro-symbolic model can generalize on unseen verb phrases and objects used in novel settings. We randomly sampled data points from the combined train and validation dataset and generated new data points. For object-level generalization, we swapped objects present in the environment with similar properties like shelf and table such that the new data point involved the usage of objects in an unseen context. For instance, the dataset had instructions to move pillows from shelf to couch and vice-versa, but the model had never seen the agent move pillows to any other object like a table. So we swapped all instances of ``couch" with ``table" and generated data points where the instruction asks the agent to move pillows from shelf to table. Similarly, other object pairs like coffee and milk, book and cd etc. were swapped in the environment to generate new data points to test object-level generalization.

For verb-level generalization, we generated a dataset following a similar approach as the object-level dataset. Sampling datapoints from the train + validation set, we replace verb frames with unseen synonyms of the same verb. For instance, we changed the verb ``boil" to ``heat" for instructions like ``boil water in the kettle" and ``turn on" to ``switch on" for instructions like ``turn on the television."

Table 2 above shows the performance comparison between \cite{She2016IncrementalAO} baseline and GoalNet Model. It is clearly seen that \cite{She2016IncrementalAO} cannot generalise to objects in unseen contexts and new verb frames without any human intervention however, GoalNet manages to generalize well on novel objects and verbs to some extent. This is mainly because of the way input is being encoded in our proposed neuro-symbolic model by incorporating conceptNet embeddings for object nodes. 

\begin{table}[t]
    \caption{Generalization results}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lcccccc@{}}
    \toprule
    \textbf{Model} & \textbf{SJI} & \textbf{IED} & \textbf{F1} & \textbf{GRR}\tabularnewline
    \midrule
    \textbf{Object Level}\tabularnewline
    \midrule
    Baseline & 0.531 & 0.467  & 0.584  & 0.471 \tabularnewline

    GOALNet & 0.203 & 0.258  & 0.270 & 0.220 \tabularnewline
    \midrule
    \textbf{Verb Level}\tabularnewline
    \midrule
    Baseline & 0.134  & 0.137 & 0.146 & 0.138 \tabularnewline
    GOALNet &  0.325 & 0.376  & 0.403 & 0.228 \tabularnewline
    \midrule
    \textbf{Paraphrasing}\tabularnewline
    \midrule
    Baseline & 0.124 & 0.127 & 0.136  &  0.128\tabularnewline
    GOALNet & 0.318 & 0.360 & 0.398 & 0.212 \tabularnewline
    \midrule
    \bottomrule
    \end{tabular}}
    \label{tab:my_label}
\end{table}

\begin{table*}[t]
    
    \centering
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{p{1in}p{2in}p{2in}}
    \toprule
    \textbf & \textbf{ACL} & \textbf{\modelname} \tabularnewline
    \midrule
    \multicolumn{3}{l}{\textbf{Put chocolate and vanilla syrup on top}} \tabularnewline
    IED& 0.0& 0.714\tabularnewline
    SJI& 0.125& 0.714\tabularnewline
    \hdashline
    Predicted Constraint positive & (grasping robot syrup\_1)(state syrup\_1 ramen)(in ramen\_1 syrup\_1)& (state mug\_1 chocolate)', '(on spoon\_1 fridge)', '(near robot beer\_1)', '(grasping robot mug\_1)', '(grasping robot syrup\_2)' \tabularnewline
    \hdashline
    Predicted constraint negative & (on syrup\_1 stovefire\_2) & (grasping robot spoon\_1)', '(on syrup\_2 stovefire\_2)'\tabularnewline
    \hdashline
    Predicted actions & moveto(ramen\_1), grasp(ramen\_1), moveto(syrup\_1), grasp(syrup\_1), add(ramen\_1 syrup\_1) & moveto mug\_1', 'grasp mug\_1', 'moveto syrup\_2', 'moveto beer\_1', 'on\_keep spoon\_1 fridge', 'grasp syrup\_2', 'squeeze syrup\_2 mug\_1'	\tabularnewline
    \midrule
    \multicolumn{3}{l}{\textbf{put pillows onto the coaches}} \tabularnewline
    IED& 0.0& 0.33\tabularnewline
    SJI& 0.076& 0.363\tabularnewline
     \hdashline
    Predicted Constraint positive & (grasping robot pillow\_1)(state pillow\_1 cd)(in cd\_1 pillow\_1) & (near robot loveseat\_1)', '(on pillow\_3 loveseat\_1)', '(grasping robot pillow\_1)', '(near robot pillow\_1)'	 \tabularnewline
     \hdashline
    Predicted constraint negative & (on pillow\_1 shelf\_1)(on cd\_1 snacktable\_1) 	 & (on pillow\_3 shelf\_1)', '(on pillow\_1 shelf\_1)'	\tabularnewline
    \hdashline
    Predicted actions & mmoveto(cd\_1), grasp(cd\_1), moveto(pillow\_1), grasp(pillow\_1), insert(cd\_1 pillow\_1)  & moveto pillow\_3', 'moveto pillow\_1', 'grasp pillow\_1', 'moveto pillow\_1', 'grasp pillow\_3', 'moveto loveseat\_1', 'on\_keep pillow\_3 loveseat\_1'	\tabularnewline
    \bottomrule
    \end{tabular}
    \caption{Qualitative results; Comparision of model prediction with \citep{She2016IncrementalAO}}
    \label{tab:my_label}
\end{table*}
 \end{itemize}





%%% ATTIC 
\iffalse
acl 16 baseline\\
our model training\\ 
ablation\\
what level of planner is needed\\
generalisation\\
length of deltag and accuracy\\
\fi
